Sovereignty of the Apps: There's more to Relevance than Downloads

The value of mobile apps is traditionally measured by metrics such as the number of downloads, installations, or user ratings. A problem with these measures is that they reflect actual usage at most indirectly. Indeed, analytic companies have suggested that retention rates, i.e., the number of days users continue to interact with an installed app are low. We conduct the first independent and large-scale study of retention rates and usage behavior trends in the wild. We study their impact on a large-scale database of app-usage data from a community of 339,842 users and more than 213,667 apps. Our analysis shows that, on average, applications lose 70% of their users in the first week, while very popular applications (top 100) lose only 45%. It also reveals, however, that many applications have more complex usage behavior patterns due to seasonality, marketing, or other factors. To capture such effects, we develop a novel app-usage behavior trend measure which provides instantaneous information about the "hotness" of an application. We identify typical trends in app popularity and classify applications into archetypes. From these, we can distinguish, for instance, trendsetters from copycat apps. In our results, roughly 40% of all apps never gain more than a handful of users. Less than 0.4% of the remaining 60% are constantly popular, 1% flop after an initial steep rise, and 7% continuously rise in popularity. We conclude by demonstrating that usage behavior trend information can be used to develop better mobile app recommendations. With the proposed usage-based measures (retention and trend), we are able to shift sovereignty in app recommendations back to where it really matters: actual usage statistics, in contrast to download count and user ratings which are prone to manipulation by people.

==> acknowledgments.tex <==
This research was partially supported by the Academy of Finland grant 277498. The work of Ella Peltonen has been supported by Doctoral School of Computer Science (DoCS). 
The publication only reflects the authors' views.
The authors are grateful to Paula Lehtola for help with Google Play data.

==> categories.tex <==
\section{Application functionality}

A common case where recommendations are needed includes a usage context: whether the user wants to play a game of some type or is looking for a better tool to perform a task. 
For a practical recommendation system, we require knowledge on the type of the applications.
This is used in order to recommend another application of similar type but with superior properties.
For instance, we might want to suggest a {\em TOP} instead of a {\em FLOP} within the same functional category.

From Google Play the app descriptions are easy to crawl by the application package name in the URL.
We fetched descriptions of \playapps{} Android applications from the Google Play store, which are also present in the Carat dataset~\cite{caratSensys2013}.
We mined these documents for the application categories, and obtained \cats{} leaf categories for applications.
Even if the trend filtering can be applied for any kind of application regardless of the language of its description, we choose to use the Android English subset in the latter part of our work.
For this set, we are able to compute their usage history and trend profile. 

\begin{table}
[!ht]
\begin{tabular}{l p{60mm}}
\textbf{Category} & \textbf{Topic description} \\
Finance & Financial tools and stock tickers \\
Photography & Camera, publishing and retouching applications \\
... & ... \\
Board & Board and card games \\
Educational & Educational games\\

\end{tabular}
\caption{Some Google Play categories for the \playapps{} apps considered in this paper}
\label{tab:topics}
\end{table}

==> funcs.tex <==
\section{Application functionality}

A common case where recommendations are needed includes a usage context: whether the user wants to play a game of some type or is looking for a better tool to perform a task. 
For a practical recommendation system, we require knowledge on the type of the applications.
This is used in order to recommend another application of similar type but with superior properties.
For instance, we might want to suggest a {\em TOP} instead of a {\em FLOP} within the same functional category.

From Google Play the app descriptions are easy to crawl by the application package name in the URL.
We fetched descriptions of 121,214 Android applications from the Google Play store, which are also present in the Carat dataset~\cite{caratSensys2013}.
From those, 106,445 had English descriptions. 
Even if the trend filtering can be applied for any kind of application regardless of the language of its description, we choose to use the Android English subset in the latter part of our work.
For this set, we are able to compute their usage history and trend profile. 

The categorization of the application in the Google Play only includes some limited knowledge, especially for the apps that are not games. To create more specific categories, we took the app descriptions from the Google Play, totally including 370,282 different words, and run topic modeling with them. We choose to use latent Dirichlet allocation (LDA) that is a well-known topic modeling algorithm~\cite{lda-orig}. It is benefited earlier~\cite{gorla-icse-14} to create categories (or topics) from Google Play and cluster the mobile applications. 

We run the LDA analysis with $K=50$. Some selected topics from those we have found from our data are presented in Table~\ref{tab:topics}.

\begin{table}
[!ht]
\begin{tabular}{p{5mm} p{60mm}}
\textbf{K} & \textbf{Topic description} \\
4 & Small games: raffle, sudoku, etc. \\
9 & Camera and video \\
15 & Adult entertainment \\
28 & Lifestyle and cooking \\
29 & Radio and music \\
33 & Language learning \\
45 & Flowers, health, and beauty\\
47 & Birdwatching, asthma, and acupuncture \\
48 & Home doctor\\

\end{tabular}
\caption{Some topics from LDA analysis of 106,445 Android applications}
\label{tab:topics}
\end{table}

==> problem.tex <==
\section{Of Relevance and Downloads}
\label{sec:dl}

\begin{figure}
	\subfloat[App \lac{}s]{\includegraphics[width=.48\columnwidth]{Figures/TrendTemplates4.png} \label{figureLifecycleA}}\hfill
	\subfloat[Example Shooting Stars]{\includegraphics[width=.48\columnwidth]{Figures/cluster_0_TOP-2.png} \label{figureLifecycleB}}
	% plot "cluster_0_com.cheetah.flashlightandroid.txt" title "com.cheetah.flashlightandroid" pointtype 9 pointsize 6, "cluster_0_com.askfm.txt" title "com.askfm" pointtype 7 pointsize 6, "cluster_0_com.icenta.sudoku.ui.txt" title "com.icenta.sudoku.ui" pointtype 5 pointsize 6
	
	\subfloat[Example Flops]{\includegraphics[width=.48\columnwidth]{Figures/category3_cluster_2_FLOP-4.png} \label{figureLifecycleC}}\hfill
	% plot "cluster_1_com.michaelpardo.ringdimmer.free.txt" pointtype 9 pointsize 5 title "com.michaelpardo.ringdimmer.free", "cluster_1_com.joaomgcd.intents.lite.txt" pointtype 7 pointsize 5 title "com.joaomgcd.intents.lite", "cluster_1_com.blogspot.droider01.stopWatchFree.txt" pointtype 5 pointsize 5 title "com.blogspot.droider01.stopWatchFree"
	\subfloat[Example Pops]{\includegraphics[width=.48\columnwidth]{Figures/cluster_2_HIGH-2.png} \label{figureLifecycleD}}
	% plot "cluster_2_com.mobilesrepublic.appygeek.txt" title "com.mobilesrepublic.appygeek" pointtype 9 pointsize 6, "cluster_2_com.mridang.hotspot.txt" title "com.mrindang.hotspot" pointtype 7 pointsize 6, "cluster_2_com.bccard.mcardapp.txt" title "com.bccard.mcardapp" pointtype 5 pointsize 6
	%  \includegraphics[width=\textwidth]{Figures/performanceInCluster.png}
	\caption{App \lac{}s with example apps (Placeholder with example figures -- to be replaced)}
	\label{figureLifecycle}
\end{figure}

In current app markets, such as Google Play and Apple's App Store,
app popularity, and indeed, relevance, is measured by simply the download count.
In addition, reaching the top ten of downloads in its category in a short time, such as a week or a month,
allows an app to be featured on the store front page.

After the initial peak, the app will not be featured any more, and may not be visible in the first page of results
for its category if it did not attain a very large user base during the launch period.
Similarly, apps are rated using 1 to 5 stars. Apps with a high rating and a high number of users who rated it are ranked first,
and apps with a low number of ratings are left in the long tail.

The above system results in popular apps gaining popularity, and less popular apps having a hard time
reaching that popularity unaided. Pestering app users to rate the app and launching large advertisement
campaigns helps app popularity, so larger organizations are much more likely to keep their apps popular.
Meanwhile, small, amazing apps that do one thing well may be left in the dust, if their budget is low and audience small.

There's more to app relevance than downloads. The typical app lifecycle has its ups and downs, as can be seen
in \fig{figureLifecycleA}.
Apps that are quickly losing their users,  no matter how many downloads they have, may be abandoned by their developers
in favor of their other, more successful apps (see \fig{figureLifecycleC}).
Applications with a small number of satisfied users can grow
quickly without advertising, but still be dwarfed by the Facebooks and Angry Birds of the market (see \fig{figureLifecycleB})).

With trend mining techniques in Section~\ref{sec:trends}, we detect whether applications are gaining, losing, or
holding their user base, and at which stage of the life cycle the app is. This allows us to predict whether
an app will stay relevant, gain traction, or possibly disappear in the near future.
